Parameterized Synthesis Case Study: AMBA AHB (extended version)

We revisit the AMBA AHB case study that has been used as a benchmark for several reactive syn- thesis tools. Synthesizing AMBA AHB implementations that can serve a large number of masters is still a difficult problem. We demonstrate how to use parameterized synthesis in token rings to obtain an implementation for a component that serves a single master, and can be arranged in a ring of arbitrarily many components. We describe new tricks -- property decompositional synthesis, and direct encoding of simple GR(1) -- that together with previously described optimizations allowed us to synthesize the model with 14 states in 30 minutes.

==> solutions.tex <==
%!TEX root = main.tex

